Consensus of hierarchical multi-agent systems with a time-varying set of active agents

Time-varying hierarchical multi-agent systems are common in many applications. A well-known solution to control these systems is to use state feedback controllers that depend on the adjacency matrix to reach consensus. This solution has been applied so far to multi-agent systems with fixed or time-varying communication topologies. In this paper, we consider single-integrator multi-agent systems where only a subset of the agents are active at any given time and the set of active agents is time-varying. This type of multi-agent system is relevant in applications such as modular multilevel converters and water pumping systems. We develop a switching algorithm that periodically selects a set of active agents through a set of graphs that connect the follower agents with a leader agent. We further prove that the developed switching algorithm combined with a classic consensus protocol yields convergence to a consensus state defined by the leader despite a time-varying set of active agents. The effectiveness of the switching algorithm is illustrated in two benchmark examples: a modular multilevel converter and a water pumping system.

==> Backup/name.tex <==
The proof of Theorem~\ref{prop:convergence} is divided into two stages. First, we must prove that the closed loop system with the switching algorithm reaches a consensus value asymptotically. Lemma 3.9 from \citep{wolfowitz1963} is essential for demonstrating that, since it proves under certain conditions, the existence of a spanning tree is sufficient for consensus under dynamically changing interaction topologies. Secondly, we need to show that the consensus value is the leader's state using Lemma 3.1 from \citep{Lunze2019} regarding the invariant property of consensus dynamics. 

% First step:

Consider a system with the agent dynamics as \eqref{eq:follower_dynamics} and \eqref{eq:leader_dynamics}, a controller as \eqref{eq:consensus_protocol} and the switching algorithm from  \eqref{eq:switching_piece_weise_d}, then a closed-loop system dynamics is defined as 

\begin{rem}
\label{rmk:primitive_condition_matrix}
Due to \eqref{eq:consensus_protocol_tunning}, as long as $ {\mathcal{G}^{'}_{i}(k)} $ has a spanning tree, \eqref{eq:defintion_of_time_varying_p_42} is primitive row-stochastic, meaning that $\boldsymbol{\mathcal{P}} (k)$ is nonnegative and has positive diagonal elements. That can easily observed if \eqref{eq:defintion_of_time_varying_p_42} is rewritten as $\boldsymbol{\mathcal{P}} (k) = \mathbf{I}_{N+1} - w k_{fb}  {\mathcal{D}}(k) + w k_{fb}  {\mathcal{A}}(k)$.  All primitive row-stochastic matrices have an invariant path to the steady-state, i.e.
\begin{equation}
    \label{eq:sia_convegence_condition}
    \lim_{n\rightarrow\infty}{\left(\mathcal{P}\right)}^{n} =  \mathbf{1}_{n} c^{\top},
\end{equation} 
\end{rem}
where $\mathcal{P} \in \mathbb{R}^{n\times n}$ is primitive row-stochastic matrix of dimension $n$ and $c \in \mathbb{R}^{n}$ is a column vector, see \citep{wolfowitz1963}.

Knowing that $\boldsymbol{\Bar{\mathcal{G}}}$ has a spanning three, using Lemma~\ref{lmm:union_graphs_convergence} and Remark~\ref{rmk:primitive_condition_matrix}, we can infer that \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} will have an invariant path as in \eqref{eq:sia_convegence_condition} and a reach consensus value consequently. The previous statement is verified in three steps: 

\begin{enumerate}
    \item Represent \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} as an infinite sequence $x_k  \in  \mathbb{R}^{N+1}$, i.e.
    \begin{equation}
    \label{eq:sequence_system_}
        x_0 =  \boldsymbol{x}(0), \quad x_{k+1} =  \boldsymbol{\mathcal{P}} (k) x_{k} \quad  \text{with} \;\, k \in \mathbb{N}_{+}.
    \end{equation}
    \item Since $\boldsymbol{\mathcal{P}} (k)$ has a periodic behaviour, due to \eqref{eq:switching_piece_weise_d}, decompose $x_k$ in a finite number of subsequences $b^{i}_{n}$, such that  
    \begin{equation}
        \label{eq:union_of_subsequence}
        x_{k} = \bigcup_{i=0}^{p-2} b^{i}_{n}
    \end{equation}
    with 
    \begin{equation}
        \label{eq:subsequence_definition}
        \begin{aligned}
            b^{0}_{n} &= \{x_0, x_{(p-1)}, x_{(p-1)2}, \ldots, x_{(p-1)\infty}\} \\ &= x_{(p-1)n}, \\
            b^{1}_{n} &= \{x_1, x_{(p-1)+1}, x_{(p-1)2+2}, \ldots, x_{(p-1)\infty +1}\} \\&= x_{(p-1)n + 1}, \\
            b^{2}_{n} &= \{x_2, x_{(p-1)+1}, x_{(p-1)2+2}, \ldots, x_{(p-1)\infty +2}\} \\&= x_{(p-1)n+2}, \\
            \vdots  \\
            b^{(p-2)}_{n} &= \{x_{(p-2)}, x_{(p-1)}, x_{(p-1)2}, \ldots, x_{(p-1)\infty + (p-2)} \} \\&= x_{(p-1)n +(p-2)},
        \end{aligned}
    \end{equation}
    where $n \in \mathbb{N}$ are the sort indices of the subsequences and $p$ is the number of graphs in the set $\Phi$ as in \eqref{eq:number_of_combinations}. Notice that the $n^{\text{th}}$ element of the subsequences $b^{i}_{n}$ corresponds to the  $k^{\text{th}}$ element of the sequence $x_{k}$, such that $k = (p-1)n + i$.
    \item Rearrange the subsequences as 
    \begin{equation}
    \label{eq:subsequence_formulation_as_function_of_b}
    {b^{i}_{0}} =  x_{i}, \quad {b^{i}_{n+1}} = \overline{\mathcal{P}}_{i} \, {b^{i}_{n}}, \quad  \forall i={0, \ldots, p-2},
    \end{equation}
    where $\overline{\mathcal{P}}_{i}$ is the product of the matrices ${\mathcal{P}}_{i}$ shifted in different orders depending on $i$, like $\overline{\mathcal{P}}_{i} = {\mathcal{P}}_{i-1} \times {\mathcal{P}}_{i-2} \times \ldots \times {\mathcal{P}}_{i}$. Consequently, $\overline{\mathcal{P}}_{i}$ are primitive row-stochastic matrices, since $$\overline{\mathcal{P}}_{i} = \mathbf{I}_{N+1} -w \cdot k_{fb} \cdot {f_{\mathcal{L}}} {\left( \boldsymbol{\Bar{\mathcal{G}}}(k)  \right)}, \;  \forall i \in\{0, \ldots, p-1\} .$$ 
    \begin{rem}
    \label{rmk:convergence_of_subsequences}
    By Lemma~\ref{lmm:union_graphs_convergence}, all the subsequences convergence to the same value, i.e.
    \begin{equation}
    \label{eq:limit_subsequences}
        \begin{aligned}
            \lim _{n \rightarrow \infty} b_{n}^{0}         &= {\underbrace{\left(\mathcal{P}_{(p-1)} \times \mathcal{P}_{(p-2)} \times \ldots \times \mathcal{P}_{0}\right)}_{\overline{\mathcal{P}}_{0}}}^{n} \cdot x_{0} \\
            \lim_{n \rightarrow \infty} {b^{1}_{n}}        &= {\underbrace{\left(\mathcal{P}_{(0)} \times \mathcal{P}_{(p-1)} \times \ldots \times \mathcal{P}_{1}\right)}_{\overline{\mathcal{P}}_{1}}}^{n} \cdot x_{1} \\
            \lim_{n \rightarrow \infty} {b^{2}_{n}}        &= {\underbrace{\left(\mathcal{P}_{(1)} \times \mathcal{P}_{(0)} \times \ldots \times \mathcal{P}_{2}\right)}_{\overline{\mathcal{P}}_{2}}}^{n} \cdot x_{2} \\
            \vdots \\
            \lim_{n \rightarrow \infty} {b^{(p-2)}_{n}}    &= {\underbrace{\left(\mathcal{P}_{(p-3)} \times \mathcal{P}_{(p-4)} \times \ldots \times \mathcal{P}_{0}\right)}_{\overline{\mathcal{P}}_{(p-2)}}}^{n} \cdot x_{(p-2)},
        \end{aligned}
    \end{equation}  
    since $$ \lim _{n \rightarrow \infty} {\overline{\mathcal{P}}_{0}}^{n} \, = \, \ldots \,  =  \, \lim_{n \rightarrow \infty} {\overline{\mathcal{P}}_{(p-2)}}^{n} \, = \,  \mathbf{1}_{N+1} c^{\top}, $$ as mentioned in Remark~\ref{rmk:primitive_condition_matrix}.
    \end{rem}
\end{enumerate}

% Second step:

From Theorem 3.5.7~\citep{Aguilar2022}, it is known that if all the subsequences of a sequence convergence to the same value, then, it can be said that the sequence converges to that value. Hence, sequence $(x_k)$ and system \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} convergence to a value that is considered the consensus value. To determine the consensus value, the invariant  property of consensus dynamics from  \citep{Lunze2019} is used. 

\begin{lem}
\label{lmm:invarint_property_consensus_dynamics}
The scalar
$$
y=\boldsymbol{w}^{\top} \boldsymbol{x}(k)
$$
is invariant under the movement of the system $\bar{\Sigma}$, where $\boldsymbol{w}^{\top} \geq 0^{\top}$ is a left eigenvector of the Laplacian matrix $\mathcal{L}$ for the vanishing eigenvalue $\lambda_1=0$.
\end{lem}

Using Lemma~\ref{lmm:invarint_property_consensus_dynamics}, for the subsequences  $b^i_n$, 
\begin{equation}
\label{eq:invariant_property_consensus_dynamics_4.2}
    y = {{\boldsymbol{w}}^{\top}} {b^{i}_{n}}, \quad \forall i=\{0, \ldots, p-2\}.
\end{equation}
Hence, $y$ is invariant for all the elements of the subsequneces, where ${{\boldsymbol{w}}^{\top}}$ is a left eigenvector of the Laplacian matrix ${\mathcal{L}}$ as in \eqref{eq:Laplacian_definition} for the eigenvalue ${\lambda_1} = 0$.
To prove \eqref{eq:invariant_property_consensus_dynamics_4.2}, we assume that there is a sequence $y_{n} =  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}}$, such that  
\begin{equation}
\label{eq:sequence_proof_invariant}
    y_{n+1}-y_{n}  = {{\boldsymbol{w}}^{\top}}{b^{i}_{n+1}} - {{\boldsymbol{w}}^{\top}}{b^{i}_{n}}, \quad \forall i=\{0, \ldots, p-2\}. 
\end{equation}
If we arrange \eqref{eq:sequence_proof_invariant} and substitute \eqref{eq:subsequence_formulation_as_function_of_b} as 
\begin{equation}
    y_{n+1} = y_{n} + {{\boldsymbol{w}}^{\top}} \left[ \; {\overline{\mathcal{P}}_{i}} {b^{i}_{n}} - {b^{i}_{n}}\right],
\end{equation}
where,  as in \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2}, $$ {\overline{\mathcal{P}}_{i}} = \mathbf{I}_{N+1} -w \cdot k_{fb} \cdot \overline{{\mathcal{L}}}_{i}.$$ Then
\begin{equation}
    \label{eq:}
    y_{n+1} = y_{n}  -w \cdot k_{fb}   \left[ {{\boldsymbol{w}}^{\top}} \; \overline{{\mathcal{L}}}_{i} \; \right] {b^{i}_{n}}.
\end{equation}

In this case, %based on remark \ref{rmk:graph_matrix_definition} that describes how the matrices $\overline{{\mathcal{L}}}_{i}$ are build, 
it can be proven that 
$${{\boldsymbol{w}}^{\top}} \overline{{\mathcal{L}}}_{i} =  \boldsymbol{0}^{\top},  \forall i \in \{0, \ldots, p-2\} \in \mathbb{N},$$
because $\overline{{\mathcal{L}}}_{i}$ represents $\boldsymbol{\Bar{\mathcal{G}}}$ as in \eqref{eq:union_switching_algorithm} \citep{Lunze2019}.  Hence, the last row of the Laplacian matrix vanishes and the matrix can be rearranged as 
$$\overline{{\mathcal{L}}}_{i} = \left(\begin{array}{c|c}
0 & \boldsymbol{0}_{N}^{\top} \\
\hline {\tilde{{\mathcal{L}}}_{i}} & l
\end{array}\right),$$
where the first row and the first column have been separated from the remaining $N$ rows and columns, $l$ is a vector such as $l^{\top} = [0\; 0\;  \ldots \; 1] \in \mathbb{N}^{N}$, ${\tilde{{\mathcal{L}}}_{i}}$ is the Laplacian matrix corresponding to the ring network that contains all the modules. Hence, two important conclusions can be derived:
\begin{enumerate}
    % \label{enum:conclusion_1}
    \item $\overline{{\mathcal{L}}}_{i}$ is triangular matrix with an eigenvalue $\lambda_1 = 0$;
    % \label{enum:conclusion_2}
    \item For these matrices, the normalised vector is defined as $\hat{{\boldsymbol{w}}}^{\top} = [ 0\;\; 0 \;\; \ldots \;\; 1]$, see \citep{Lunze2019}.
\end{enumerate} 
Using conclusion 1, it can be proven that exists a scalar $y$ as in \eqref{eq:invariant_property_consensus_dynamics_4.2}, since 
$$ y_{n+1} =  y_{n}, \quad \forall n\in \mathbb{N}_{+}.$$
Using conclusion 2, it can be proved that the subsequences converge to value determined by the leader, such as $\bar{x}  =  {x_L}$, since the invariant property of the system the scalar $y$ remains constant, i.e. 
$$ y =  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}} =  {{\boldsymbol{w}}^{\top}} {b^{i}_{0}}. $$
If the state of the leader $x_L$ is kept constant for a period of time long enough, then 
$$ {{\boldsymbol{w}}^{\top}} {b^{i}_{0}} = \lim_{n \rightarrow \infty}  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}} = {{\boldsymbol{w}}^{\top}} \bar{x} {\boldsymbol{1}_{N+1}}, \quad \forall i=\{0,\ldots,p-2\} $$
then  $$ \bar{x} = \hat{{\boldsymbol{w}}}^{\top}  {b^{i}_{0}} =   {{x}_L(0)}$$
where $$\hat{{\boldsymbol{w}}}^{\top} = \frac{1}{ {{\boldsymbol{w}}^{\top}} \boldsymbol{1}_{N+1}}  {{\boldsymbol{w}}^{\top}}.$$

\begin{rem}
\label{rmk:convergence_time_ }
Theorem~\ref{prop:convergence} only demonstrates the system's asymptotic convergence. The union of the graph $(\boldsymbol{\Bar{\mathcal{G}}})$ with a spanning tree is a necessary condition for this proof. As a result, the time difference $M$ must be large enough to allow the iteration through all of the graphs in the set $\Phi (m)$. It is also worth noting that the convergence time is affected by how we calculate $k_{fb}$.
\end{rem}The proof of Theorem~\ref{prop:convergence} is divided into two stages. First, we must prove that the closed loop system with the switching algorithm reaches a consensus value asymptotically. Lemma 3.9 from \citep{wolfowitz1963} is essential for demonstrating that, since it proves under certain conditions, the existence of a spanning tree is sufficient for consensus under dynamically changing interaction topologies. Secondly, we need to show that the consensus value is the leader's state using Lemma 3.1 from \citep{Lunze2019} regarding the invariant property of consensus dynamics. 

% First step:

Consider a system with the agent dynamics as \eqref{eq:follower_dynamics} and \eqref{eq:leader_dynamics}, a controller as \eqref{eq:consensus_protocol} and the switching algorithm from  \eqref{eq:switching_piece_weise_d}, then a closed-loop system dynamics is defined as 

\begin{rem}
\label{rmk:primitive_condition_matrix}
Due to \eqref{eq:consensus_protocol_tunning}, as long as $ {\mathcal{G}^{'}_{i}(k)} $ has a spanning tree, \eqref{eq:defintion_of_time_varying_p_42} is primitive row-stochastic, meaning that $\boldsymbol{\mathcal{P}} (k)$ is nonnegative and has positive diagonal elements. That can easily observed if \eqref{eq:defintion_of_time_varying_p_42} is rewritten as $\boldsymbol{\mathcal{P}} (k) = \mathbf{I}_{N+1} - w k_{fb}  {\mathcal{D}}(k) + w k_{fb}  {\mathcal{A}}(k)$.  All primitive row-stochastic matrices have an invariant path to the steady-state, i.e.
\begin{equation}
    \label{eq:sia_convegence_condition}
    \lim_{n\rightarrow\infty}{\left(\mathcal{P}\right)}^{n} =  \mathbf{1}_{n} c^{\top},
\end{equation} 
\end{rem}
where $\mathcal{P} \in \mathbb{R}^{n\times n}$ is primitive row-stochastic matrix of dimension $n$ and $c \in \mathbb{R}^{n}$ is a column vector, see \citep{wolfowitz1963}.

Knowing that $\boldsymbol{\Bar{\mathcal{G}}}$ has a spanning three, using Lemma~\ref{lmm:union_graphs_convergence} and Remark~\ref{rmk:primitive_condition_matrix}, we can infer that \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} will have an invariant path as in \eqref{eq:sia_convegence_condition} and a reach consensus value consequently. The previous statement is verified in three steps: 

\begin{enumerate}
    \item Represent \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} as an infinite sequence $x_k  \in  \mathbb{R}^{N+1}$, i.e.
    \begin{equation}
    \label{eq:sequence_system_}
        x_0 =  \boldsymbol{x}(0), \quad x_{k+1} =  \boldsymbol{\mathcal{P}} (k) x_{k} \quad  \text{with} \;\, k \in \mathbb{N}_{+}.
    \end{equation}
    \item Since $\boldsymbol{\mathcal{P}} (k)$ has a periodic behaviour, due to \eqref{eq:switching_piece_weise_d}, decompose $x_k$ in a finite number of subsequences $b^{i}_{n}$, such that  
    \begin{equation}
        \label{eq:union_of_subsequence}
        x_{k} = \bigcup_{i=0}^{p-2} b^{i}_{n}
    \end{equation}
    with 
    \begin{equation}
        \label{eq:subsequence_definition}
        \begin{aligned}
            b^{0}_{n} &= \{x_0, x_{(p-1)}, x_{(p-1)2}, \ldots, x_{(p-1)\infty}\} \\ &= x_{(p-1)n}, \\
            b^{1}_{n} &= \{x_1, x_{(p-1)+1}, x_{(p-1)2+2}, \ldots, x_{(p-1)\infty +1}\} \\&= x_{(p-1)n + 1}, \\
            b^{2}_{n} &= \{x_2, x_{(p-1)+1}, x_{(p-1)2+2}, \ldots, x_{(p-1)\infty +2}\} \\&= x_{(p-1)n+2}, \\
            \vdots  \\
            b^{(p-2)}_{n} &= \{x_{(p-2)}, x_{(p-1)}, x_{(p-1)2}, \ldots, x_{(p-1)\infty + (p-2)} \} \\&= x_{(p-1)n +(p-2)},
        \end{aligned}
    \end{equation}
    where $n \in \mathbb{N}$ are the sort indices of the subsequences and $p$ is the number of graphs in the set $\Phi$ as in \eqref{eq:number_of_combinations}. Notice that the $n^{\text{th}}$ element of the subsequences $b^{i}_{n}$ corresponds to the  $k^{\text{th}}$ element of the sequence $x_{k}$, such that $k = (p-1)n + i$.
    \item Rearrange the subsequences as 
    \begin{equation}
    \label{eq:subsequence_formulation_as_function_of_b}
    {b^{i}_{0}} =  x_{i}, \quad {b^{i}_{n+1}} = \overline{\mathcal{P}}_{i} \, {b^{i}_{n}}, \quad  \forall i={0, \ldots, p-2},
    \end{equation}
    where $\overline{\mathcal{P}}_{i}$ is the product of the matrices ${\mathcal{P}}_{i}$ shifted in different orders depending on $i$, like $\overline{\mathcal{P}}_{i} = {\mathcal{P}}_{i-1} \times {\mathcal{P}}_{i-2} \times \ldots \times {\mathcal{P}}_{i}$. Consequently, $\overline{\mathcal{P}}_{i}$ are primitive row-stochastic matrices, since $$\overline{\mathcal{P}}_{i} = \mathbf{I}_{N+1} -w \cdot k_{fb} \cdot {f_{\mathcal{L}}} {\left( \boldsymbol{\Bar{\mathcal{G}}}(k)  \right)}, \;  \forall i \in\{0, \ldots, p-1\} .$$ 
    \begin{rem}
    \label{rmk:convergence_of_subsequences}
    By Lemma~\ref{lmm:union_graphs_convergence}, all the subsequences convergence to the same value, i.e.
    \begin{equation}
    \label{eq:limit_subsequences}
        \begin{aligned}
            \lim _{n \rightarrow \infty} b_{n}^{0}         &= {\underbrace{\left(\mathcal{P}_{(p-1)} \times \mathcal{P}_{(p-2)} \times \ldots \times \mathcal{P}_{0}\right)}_{\overline{\mathcal{P}}_{0}}}^{n} \cdot x_{0} \\
            \lim_{n \rightarrow \infty} {b^{1}_{n}}        &= {\underbrace{\left(\mathcal{P}_{(0)} \times \mathcal{P}_{(p-1)} \times \ldots \times \mathcal{P}_{1}\right)}_{\overline{\mathcal{P}}_{1}}}^{n} \cdot x_{1} \\
            \lim_{n \rightarrow \infty} {b^{2}_{n}}        &= {\underbrace{\left(\mathcal{P}_{(1)} \times \mathcal{P}_{(0)} \times \ldots \times \mathcal{P}_{2}\right)}_{\overline{\mathcal{P}}_{2}}}^{n} \cdot x_{2} \\
            \vdots \\
            \lim_{n \rightarrow \infty} {b^{(p-2)}_{n}}    &= {\underbrace{\left(\mathcal{P}_{(p-3)} \times \mathcal{P}_{(p-4)} \times \ldots \times \mathcal{P}_{0}\right)}_{\overline{\mathcal{P}}_{(p-2)}}}^{n} \cdot x_{(p-2)},
        \end{aligned}
    \end{equation}  
    since $$ \lim _{n \rightarrow \infty} {\overline{\mathcal{P}}_{0}}^{n} \, = \, \ldots \,  =  \, \lim_{n \rightarrow \infty} {\overline{\mathcal{P}}_{(p-2)}}^{n} \, = \,  \mathbf{1}_{N+1} c^{\top}, $$ as mentioned in Remark~\ref{rmk:primitive_condition_matrix}.
    \end{rem}
\end{enumerate}

% Second step:

From Theorem 3.5.7~\citep{Aguilar2022}, it is known that if all the subsequences of a sequence convergence to the same value, then, it can be said that the sequence converges to that value. Hence, sequence $(x_k)$ and system \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2} convergence to a value that is considered the consensus value. To determine the consensus value, the invariant  property of consensus dynamics from  \citep{Lunze2019} is used. 

\begin{lem}
\label{lmm:invarint_property_consensus_dynamics}
The scalar
$$
y=\boldsymbol{w}^{\top} \boldsymbol{x}(k)
$$
is invariant under the movement of the system $\bar{\Sigma}$, where $\boldsymbol{w}^{\top} \geq 0^{\top}$ is a left eigenvector of the Laplacian matrix $\mathcal{L}$ for the vanishing eigenvalue $\lambda_1=0$.
\end{lem}

Using Lemma~\ref{lmm:invarint_property_consensus_dynamics}, for the subsequences  $b^i_n$, 
\begin{equation}
\label{eq:invariant_property_consensus_dynamics_4.2}
    y = {{\boldsymbol{w}}^{\top}} {b^{i}_{n}}, \quad \forall i=\{0, \ldots, p-2\}.
\end{equation}
Hence, $y$ is invariant for all the elements of the subsequneces, where ${{\boldsymbol{w}}^{\top}}$ is a left eigenvector of the Laplacian matrix ${\mathcal{L}}$ as in \eqref{eq:Laplacian_definition} for the eigenvalue ${\lambda_1} = 0$.
To prove \eqref{eq:invariant_property_consensus_dynamics_4.2}, we assume that there is a sequence $y_{n} =  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}}$, such that  
\begin{equation}
\label{eq:sequence_proof_invariant}
    y_{n+1}-y_{n}  = {{\boldsymbol{w}}^{\top}}{b^{i}_{n+1}} - {{\boldsymbol{w}}^{\top}}{b^{i}_{n}}, \quad \forall i=\{0, \ldots, p-2\}. 
\end{equation}
If we arrange \eqref{eq:sequence_proof_invariant} and substitute \eqref{eq:subsequence_formulation_as_function_of_b} as 
\begin{equation}
    y_{n+1} = y_{n} + {{\boldsymbol{w}}^{\top}} \left[ \; {\overline{\mathcal{P}}_{i}} {b^{i}_{n}} - {b^{i}_{n}}\right],
\end{equation}
where,  as in \eqref{eq:overall_system_fedback_controller_discrete_time_varying_4.2}, $$ {\overline{\mathcal{P}}_{i}} = \mathbf{I}_{N+1} -w \cdot k_{fb} \cdot \overline{{\mathcal{L}}}_{i}.$$ Then
\begin{equation}
    \label{eq:}
    y_{n+1} = y_{n}  -w \cdot k_{fb}   \left[ {{\boldsymbol{w}}^{\top}} \; \overline{{\mathcal{L}}}_{i} \; \right] {b^{i}_{n}}.
\end{equation}

In this case, %based on remark \ref{rmk:graph_matrix_definition} that describes how the matrices $\overline{{\mathcal{L}}}_{i}$ are build, 
it can be proven that 
$${{\boldsymbol{w}}^{\top}} \overline{{\mathcal{L}}}_{i} =  \boldsymbol{0}^{\top},  \forall i \in \{0, \ldots, p-2\} \in \mathbb{N},$$
because $\overline{{\mathcal{L}}}_{i}$ represents $\boldsymbol{\Bar{\mathcal{G}}}$ as in \eqref{eq:union_switching_algorithm} \citep{Lunze2019}.  Hence, the last row of the Laplacian matrix vanishes and the matrix can be rearranged as 
$$\overline{{\mathcal{L}}}_{i} = \left(\begin{array}{c|c}
0 & \boldsymbol{0}_{N}^{\top} \\
\hline {\tilde{{\mathcal{L}}}_{i}} & l
\end{array}\right),$$
where the first row and the first column have been separated from the remaining $N$ rows and columns, $l$ is a vector such as $l^{\top} = [0\; 0\;  \ldots \; 1] \in \mathbb{N}^{N}$, ${\tilde{{\mathcal{L}}}_{i}}$ is the Laplacian matrix corresponding to the ring network that contains all the modules. Hence, two important conclusions can be derived:
\begin{enumerate}
    % \label{enum:conclusion_1}
    \item $\overline{{\mathcal{L}}}_{i}$ is triangular matrix with an eigenvalue $\lambda_1 = 0$;
    % \label{enum:conclusion_2}
    \item For these matrices, the normalised vector is defined as $\hat{{\boldsymbol{w}}}^{\top} = [ 0\;\; 0 \;\; \ldots \;\; 1]$, see \citep{Lunze2019}.
\end{enumerate} 
Using conclusion 1, it can be proven that exists a scalar $y$ as in \eqref{eq:invariant_property_consensus_dynamics_4.2}, since 
$$ y_{n+1} =  y_{n}, \quad \forall n\in \mathbb{N}_{+}.$$
Using conclusion 2, it can be proved that the subsequences converge to value determined by the leader, such as $\bar{x}  =  {x_L}$, since the invariant property of the system the scalar $y$ remains constant, i.e. 
$$ y =  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}} =  {{\boldsymbol{w}}^{\top}} {b^{i}_{0}}. $$
If the state of the leader $x_L$ is kept constant for a period of time long enough, then 
$$ {{\boldsymbol{w}}^{\top}} {b^{i}_{0}} = \lim_{n \rightarrow \infty}  {{\boldsymbol{w}}^{\top}} {b^{i}_{n}} = {{\boldsymbol{w}}^{\top}} \bar{x} {\boldsymbol{1}_{N+1}}, \quad \forall i=\{0,\ldots,p-2\} $$
then  $$ \bar{x} = \hat{{\boldsymbol{w}}}^{\top}  {b^{i}_{0}} =   {{x}_L(0)}$$
where $$\hat{{\boldsymbol{w}}}^{\top} = \frac{1}{ {{\boldsymbol{w}}^{\top}} \boldsymbol{1}_{N+1}}  {{\boldsymbol{w}}^{\top}}.$$

\begin{rem}
\label{rmk:convergence_time_ }
Theorem~\ref{prop:convergence} only demonstrates the system's asymptotic convergence. The union of the graph $(\boldsymbol{\Bar{\mathcal{G}}})$ with a spanning tree is a necessary condition for this proof. As a result, the time difference $M$ must be large enough to allow the iteration through all of the graphs in the set $\Phi (m)$. It is also worth noting that the convergence time is affected by how we calculate $k_{fb}$.
\end{rem}




